An Information-Theoretic Justification for Model Pruning

We study the neural network (NN) compression problem, viewing the tension between the compression ratio and NN performance through the lens of rate-distortion theory. We choose a distortion metric that reflects the effect of NN compression on the model output and derive the tradeoff between rate (compression) and distortion. In addition to characterizing theoretical limits of NN compression, this formulation shows that \emph{pruning}, implicitly or explicitly, must be a part of a good compression algorithm. This observation bridges a gap between parts of the literature pertaining to NN and data compression, respectively, providing insight into the empirical success of model pruning. Finally, we propose a novel pruning strategy derived from our information-theoretic formulation and show that it outperforms the relevant baselines on CIFAR-10 and ImageNet datasets.

==> sections/02-prelims.tex <==
\section{Preliminaries}
\label{prelims}
In this section, we present the problem setup, briefly introduce the rate distortion theory and successive refinement, and empirically show that NN weights can be modelled by a Laplace distribution. 

\subsection{Problem Statement and Notation}
\label{pre_density}
We study a supervised learning problem where NN parameters $w$ are trained to learn a conditional distribution $p_w(y|x)$ of labels $y$ given the inputs $x$. During the training, the model has access to samples $\mathcal{D} = \{(x_i, y_i)\}_{i=1}^m$ drawn from the data distribution $(x,y) \sim p_{x,y}$. The performance metric in our learning problem is the accuracy of the prediction $p_w(y|x)$ on the test data drawn from the same distribution $p_{x,y}$. We aim to compress $w$ to represent the model with the minimum number of bits while preserving the accuracy of the model. %\noa{How about ``... minimum number of bits while minimizing the distortion of the weights''.} 
This is a lossy compression problem where the distortion is a measure of the distance between the original model and compressed model, and the rate is the number of bits required to represent one weight. In information-theoretic term, rate distortion theory characterizes the minimum achievable rate given the target distortion.
%In information theory, the lower bound of the rate given a distortion is formulated via rate distortion theory. 

%As an example, suppose there is a source that produces the sequence $U_1, \dots, U_n$ i.i.d. $\sim p(u)$, $u \in \mathcal{U}$.}
More precisely, let $\bU_1, \dots, 
\bU_n\in\mathcal{U}$ be a source sequence generated by i.i.d. $\sim p(u)$. The encoder $f_e: \mathcal{U}^n \rightarrow  \{0,1\}^{nR}$ describes this sequence in $nR$ bits, where this binary representation is called a ``message'' $m$.
The decoder $f_d: \{0,1\}^{nR} \rightarrow \hat{\mathcal{U}}^n$ reconstructs an estimate $\hat{u}^{n} \in \hat{\mathcal{U}}^n$ based on $m\in\{0,1\}^{nR}$. This process, summarized in Figure~\ref{fig:enc_dec_diagram}(a), is called source coding. 
\begin{figure}[h!]
        \centering 
        \subfigure[Source Coding.]{\includegraphics[width=.45\textwidth]{figures/Succ_refin_1_dec.png}}
        \subfigure[Successive Refinement. ]{\includegraphics[width=.45\textwidth]{figures/Succ_refin_2_dec_u2.png}}
       \caption{(a) Source Coding, (b) Successive Refinement with $2$ Decoders.}
       \label{fig:enc_dec_diagram}
       \end{figure}
%\noa{I prefer $nR_1$ instead of $R_1n$, but it is not critical.}

The number of bits per source symbol %$u$\noa{instead of using $u$, how about ``The number of bits per source symbol ...''} 
($\frac{nR}{n}=R$ in this case) and the ``distance'' %\noa{(distortion)}
$D(u^n, \hat{u}^n)=\sum_{(u,\hat{u})}d(u,\hat{u})$ between $u^n $ and $\hat{u}^n$ are named as rate and distortion, respectively. Ideally, we would like to keep both rate and distortion low, but there is a trade-off between these two quantities, which is characterized by the rate-distortion function \cite{shannon2001mathematical, berger2003rate, elements_of_it} as:
%$f_e: \mathcal{U}^n \rightarrow  \mathcal{B}^{Rn}$ where $b^{Rn} \in B^{Rn} \subseteq \{0,1\}^{Rn}$. $b_1, \dots, b_{Rn}$ is a lossy binary representation of the input $u_1, \dots, u_n$. The decoder $f_d: \mathcal{B}^{Rn} \rightarrow \hat{\mathcal{U}}^n$ reconstructs an estimate $\hat{u}^{n} \in \hat{\mathcal{U}}^n$ from the binary representation $b^{Rn}$. The rate is defined as the number of bits $b$ per symbol $u$ ($R$ in this case) and the distortion $d(u, \hat{u})$ is the cost of representing $u$ as $\hat{u}$. Ideally, we would like to keep both $R$ and $d(u, \hat{u})$ small but there is a trade off between these two quantity, which is given by the rate distortion theory as follows: \cite{shannon2001mathematical, elements_of_it}:
%{\centering
  %$ \displaystyle
\begin{equation}
\label{rd}
    R(D) = \min_{p(\hat{u}|u): \sum_{(u,\hat{u})} p(u)p(\hat{u}|u) d(u, \hat{u}) \leq D} I(\bU; \bUh)
\end{equation}
%  %$ 
%\par}
where $I(\bU;\bUh)$ is the mutual information between $\bU$ and $\bUh$, and $d(u, \hat{u})$ is a predefined distortion metric, e.g. $\ell_2$ distance. The rate-distortion function $R(D)$ in Eq.~\ref{rd} is the minimum achievable rate at distortion $D$, and the conditional distribution $p(\hat{u}|u)$
that achieves $I(\bU; \bUh) = R(D)$ explains how an optimal encoder-decoder pair should operate for the source $p(u)$.
Clearly, source distribution has a critical role in the solution of the rate distortion problem.
We discuss possible assumptions for the distribution of NN weights in the next section. 

Throughout the paper, $w \in \R^n$ is the weights of a trained model, $f_L(u;\mu, b) = \frac{1}{2b} \exp{-\frac{|u-\mu|}{b}}$ is the probability density function (pdf) of Laplace distribution with mean $\mu$ and scale $b$, $f_{\text{exp}}(u;\lambda) = \lambda e^{-\lambda u}$ is the pdf of exponential distribution with parameter $\lambda$. Logarithms are in base $2$ and rate is defined as bits per symbol. We define the compression rate as the ratio of the original model size to the compressed model's size, where size is the length of the model's binary representation.
%\noa{I prefer $f_L(u;\mu, b)$ and $f_{\text{exp}}(u;\lambda)$ since $\mu, b,\lambda$ are parameters not conditional variables.}

\subsection{Density of Neural Network Parameters}
\label{section_density}
In order to apply the rate distortion theory for NN compression, we need a good density estimation for the NN weights. Figure~\ref{fig:density_weight}(a) shows the density of ResNet-18 weights trained on CIFAR-10, and corresponding Gaussian and Laplacian distributions having the same mean and variance. While prior work assumes Gaussian distribution for the underlying distribution of NN weights \cite{gao2019rate}, Figure~\ref{fig:density_weight}(a) suggests that zero-mean Laplacian distribution is a better fit. Apart from being a better approximation to the distribution of NN weights, Laplacian distribution has another appealing property:

{\centering
  $ \displaystyle
    \begin{aligned} 
      u \sim f_L(u;\mu, b) \ \Rightarrow \ |u-\mu|\sim f_{\text{exp}}(u;\frac{1}{b}). 
    \end{aligned}
  $ 
\par}
%\noa{$f_{exp}$ above?}
That is, if $u$ is a sample from a Laplacian source with mean $\mu$ and scale $b$, then $|u-\mu|$ has an exponential distribution with parameter $\frac{1}{b}$. Figure~\ref{fig:density_weight}(b) shows that exponential distribution almost perfectly matches the magnitude of NN weights. This observation enables us to study the compression of sign-free weights by applying rate distortion theory to the exponential source. The reason why we discard sign bits follows the conclusion of \cite{isiknoisy}. They show that small perturbations on the weights may lead to sign errors that degrade the NN performance significantly. Thus, we keep the sign bits as they are and compress the sign-free weights. We refer the reader to Appendix~\ref{density_app} for density plots of ResNet-50, VGG-16, LeNet-5-Caffe, and LeNet-300-100.

\begin{figure}[h!]
        \centering %
        \subfigure[Density of Weights.]{\includegraphics[width=.2383\textwidth]{figures/weight_density_resnet18.jpg}}
        \subfigure[Density of Sign-Free Weights. ]{\includegraphics[width=.2383\textwidth]{figures/weight_density_resnet18_exp.jpg}}
    \caption{Density of ResNet-18 (a) Signed Weights, (b) Sign-free Weights. ResNet-18 is trained on CIFAR-10. Gaus: Gaussian, Lap.: Laplacian, Exp.: Exponential, Wt.: NN Weights.}\label{fig:density_weight}
   \end{figure}
   
%\berivan{should we cite \cite{si2014lossy, erez2020exponential}?}
%\noa{I think we can simply mention \cite{si2014lossy} since they provide a compression algorithm for exponential source. Their idea is applying binary compression schemes to the binary expansion of sources.They just assumed that there exists an efficient binary source compression algorithm, so their algorithm is not 100\% practical while we showed the practicality of our algorithm. Also, \cite{erez2020exponential} they considered compression with multiple descriptions which is not directly relavent to ours. You can cite both if you want to spend a paragraph about the prior works on Laplacian (exponential) source compression (which is worth it I guess but not necessary).} \berivan{i will come to that later to see how much space we have for this paragraph}



\subsection{Successive Refinement}\label{sec:successive}
%\berivan{if we have space, a diagram for successive refinement with 1 encoder, 2 decoders}
%\noa{I am not sure whether we describe more on rate distortion theory since the audiences may not be familiar with concepts like message, rate-distortion function, mutual information, etc.}
In the successive refinement problem, summarized in Figure~\ref{fig:enc_dec_diagram}(b), the encoder wants to describe the source to two decoders, where each decoder has its own target distortion, $D_1$ and $D_2$.
Instead of having separate encoding schemes for each decoder,
the successive refinement encoder encodes a message $m_1$ for Decoder 1 (with higher target distortion, $D_1$),
and encodes an extra message $m_2$ where the second decoder gets both $m_1$ and $m_2$. %\noa{Decoder 2 does not have to reconstruct $\hat{U}_2^n$ (of course it can}.\st{Both Decoder 1 and Decoder 2 reconstruct $\bUh^n_1$ from $m_1$ with distortion $D_1$.} 
Receiving both $m_1$ and $m_2$, Decoder 2 reconstructs $\bUh_2^n$ with distortion $D_2$.
%\noa{I think the sub-optimal part is crucial since successive refinability is a rare property.}
Since the message $m_1$ is re-used, the performance of successive refinement encoder is sub-optimal in general.
%However, in some cases, the successive refinement encoder achieves the optimum rate distortion trade-off as if dedicated encoders were used separately.
However, in some cases, the successive refinement encoder achieves the optimum rate distortion trade-off as if dedicated encoders were used separately.
In such a case, we call the source (distribution) and the distortion pair ``successively refinable'' \cite{koshelev1980hierarchical, equitz1991successive}.

The idea of successive refinement can be utilized to reduce the complexity of the information-theoretic optimal compression scheme.
The optimum scheme in rate distortion theory finds the message $m$ that codes the best reconstruction $\bUh$ from the codebook of size $2^{nR}$ (see Figure~\ref{fig:enc_dec_diagram}(a)).
This is not implementable in practice due to the exponential complexity.
The successive refinement encoder in Figure~\ref{fig:enc_dec_diagram}(b) can find the best reconstruction iteratively, and therefore can reduce the complexity. Instead of searching over $2^{nR}$ codewords, the successive refinement encoder finds $m_1$ that codes a sub-codeword from the sub-codebook of size
$2^{nR_1}$, and $m_2$ that codes a sub-codeword from another sub-codebook of size $2^{nR_2}$ where $R_1,R_2  \approx R/2$.
Then, the complexity in successive refinement, $2^{nR_1}+2^{nR_2}$, is smaller than that of one-step source coding, $2^{nR}$.
We can increase the number of steps (number of decoders) to reduce the complexity further.
For Gaussian source under mean squared error, which is also successively refinable,
\cite{venkataramanan2014lossy} and \cite{no2016rateless} generalize the idea of successive refinement,
and propose low complexity schemes that achieve the optimum rate distortion trade-off curve. Note that the exponential source under one-sided $\ell_1$ loss is also successively refinable.
In this paper, we propose a practical low complexity compression scheme for exponential source based on successive refinement,
which also provides a novel pruning strategy for NN compression.
%We call our method ``successive pruning'' as it performs a successive refinement of NN weights.


==> sections/03-method.tex <==
\section{Methodology}
\label{method}
In this section, we study lossy compression of exponential sources (Section~\ref{comp_exp}), and present ways to apply our findings in NN compression (Section~\ref{comp_NN}) and communication-efficient federated learning (Section~\ref{fl}) problems.  
\subsection{Compression for Exponential Source}
\label{comp_exp}
\subsubsection{Lossy Compression}

We consider i.i.d. exponential source sequence $u_1, \dots, u_n$ with distribution $f_{exp}(u;\lambda) = \lambda e^{-\lambda u}$ for $u \geq 0$, %\noa{$f_{exp}$?, also, I prefer$f_{exp}(x;\lambda)$ since $\lambda$ is a parameter not a conditional variable.} 
reconstruction $v_1, \dots, v_n$, and one-sided $\ell_1$ distortion given by:
\begin{align*}
    d(u, v) = \begin{cases} u - v, & \text{if} \ u \geq v \\
                    \infty,  & \text{otherwise.}\end{cases}
\end{align*}    
We start with the rate distortion function which is a minimum achievable rate given the target distortion $D$:

\begin{lem}{\cite{verdu1996exponential}} The rate distortion function for an exponential source with one-sided distortion is given by
\begin{align}
\begin{aligned}
    R(D) = \begin{cases} -\log(\lambda D), & \ 0 \leq D \leq \frac{1}{\lambda} \\
    0, &  D > \frac{1}{\lambda}\end{cases}
\end{aligned}
\label{eq_rd_exp}
\end{align}
with the following optimal conditional probability distribution that achieves the minimum mutual information
%this limit is another exponential distribution with parameter $1/D$:
\begin{align}
\begin{aligned}
    f_{\bU|\bV}(u|v) = \begin{cases}\frac{1}{D} e^{-(u-v)/D},& \mbox{ $u \geq v \geq 0$}\\
    0, & \mbox{ otherwise}.
    \end{cases}
\end{aligned}
\label{eq_cond_dist}
\end{align}
\label{rd_exp}
\end{lem}
%\vspace*{-1.85\baselineskip}
 Moreover, the marginal distribution of $\bV$ is as follows
\begin{align}
\begin{aligned}
f_{\bV}(v) = \lambda D \cdot \delta (v) + (1-\lambda D) \cdot \lambda e^{-\lambda v}
\end{aligned}
\label{eq:marginal}
\end{align}
where $\delta(v)$ is a Dirac measure at 0.
The proofs of Lemma~\ref{rd_exp} and Eq.~\ref{eq:marginal} are given in Appendix~\ref{comp_exp_app}. The sparsity of $\bV$ in Eq.~\ref{eq:marginal} suggests pruning as an optimal compression strategy! 

Note that the distribution of $\bU-\bV$ given $\bV=v$ is exponential with parameter $1/D$.
Based on this property, we can design an explicit successive refinement encoder. Instead of a successive refinement scheme with two decoders as described in Section \ref{sec:successive}, we consider the successive refinement problem with $L$ decoders.
Let $\lambda = \lambda_0 < \lambda_1 < \dots < \lambda_L$ where $D_t = 1/\lambda_t$ is a target distortion at the $t$-th decoder.
We begin by setting $\bU^{(0)} = u^n$.
At $t$-th iteration, the encoder finds $\bV^{(t)}$ that minimizes the distance between $D(\bU^{(t-1)}, \bV^{(t)})$ from the codebook $\cC^{(t)}$,
then computes $\bU^{(t)} = \bU^{(t-1)} - \bV^{(t)}$.
The $t$-th codebook consists of codewords generated by the marginal distribution in Eq.~\ref{eq:marginal}:
%of i.i.d. random variables with distribution
\begin{align*}
f_{\bV^{(t)}}(v) = \frac{\lambda_{t-1}}{\lambda_{t}} \cdot \delta (v) + \left(1-\frac{\lambda_{t-1}}{\lambda_{t}}\right) \cdot \lambda_{t-1}e^{-\lambda_{t-1} v}
\end{align*}
Since $\bU^{(t)}$ is an i.i.d.\ exponential random sequence from Eq.~\ref{eq_cond_dist}, the encoder can keep applying the compression schemes for exponential sources at each iteration.
At iteration $t$, the reconstruction on the decoder side is $\bUh^{(t)} = \sum_{\tau=1}^t \bV^{(\tau)}$. 
%\begin{align*}
%\bUh^{(t)} = \sum_{\tau=1}^t \bV^{(\tau)}.
%\end{align*}
In summary, for $1\leq t\leq L$, the original information-theoretic successive refinement encoder performs the following steps iteratively:
\begin{enumerate}
\item Find $\bV^{(t)}\in\cC^{(t)}$ that minimizes $D(\bU^{(t-1)}, \bV^{(t)})$.
\item Update $\bf U$ as ${\bf U}^{(t)} = \bU^{(t-1)} - \bV^{(t)}$.
\end{enumerate}
We further simplify the above algorithm by a heuristic approach which does not require to generate random codewords or compute the distortion between $\bU^{(t-1)}$ and $\bV^{(t)}$ at each iteration. The heuristic coding scheme is as follows:
% Lemma~\ref{rd_exp} states that once the decoder has the distorted variable $\hat{u}$ that achieves the $R(D)$ limit, the missing (lost) information about $u$ given $\hat{u}$ is again exponentially distributed. This will be useful in the construction of our successive refinable coding scheme. An important question for us is how to reconstruct $\hat{u}$ that achieves the limit in Eq.~\ref{eq_rd_exp}. \\

% \begin{thm}
% The rate distortion function for an exponential source with one-sided distortion (Eq.~\ref{eq_rd_exp}) is achieved with $\hat{U}$ distributed according to the following distribution:
% \begin{align}
%     \begin{aligned}
%     f_{\hat{U}}(\hat{u}) = \lambda D \cdot \delta (\hat{u}) + (1-\lambda D) \cdot \lambda e^{-\lambda \hat{u}}
%     \end{aligned}
% \end{align}
% \label{thm_sparse_code}
% \end{thm}
% The proof of Theorem~\ref{thm_sparse_code} is given in Appendix~\ref{comp_exp_app}.
% \noa{I think we do not have to prove  this}.
% Theorem~\ref{thm_sparse_code} suggests a sparse codebook to achieve the rate distortion limit in Eq.~\ref{eq_rd_exp}. \\

% \berivan{TODO: some connection from here to our algorithm} \\

% Then the iterative coding scheme for an $n$-dimensional i.i.d. exponential source $U^{(0)}=(U^{(0)}_1, \dots,U^{(0)}_n )$ for $t\geq 1$ is as follows:
\begin{enumerate}
    %\item Pick an index $i$ randomly from $\{j: \bU^{(t-1)}_j \geq \frac{1}{\lambda_{t-1}}\}$. Encode $i$ as $m_t$.
    \item Find index $i$ such that $\bU^{(t-1)}_i \geq \frac{1}{\lambda_{t-1}}$. If there are more than one such indices, pick an index $i$ randomly. Encode $i$ as $m_t$.
    %\noa{We have to mention that $m_t = i$ since $m_t$ appears in the following figure.}
    \item Let $\bV^{(t)}$ be an $n$-dimensional all-zero vector except $\bV^{(t)}_i = \frac{1}{\lambda_{t-1}}$.
    \item Let $\bU^{(t)} = \bU^{(t-1)} - \bV^{(t)}$.
    \item Set $\lambda_t = \frac{n}{n-1} \cdot \lambda_{t-1}$.
\end{enumerate}

\begin{figure}[t!]
        \centering 
        \resizebox{\columnwidth}{!}{
        \includegraphics[]{figures/succ_prun_iterations_concise.png}}
        %\includegraphics[width=.48\textwidth]{figures/succ_prun_iterations_concise.png}}
       \caption{Successive Pruning. E: Encoder, D: Decoder.}
       \label{fig:succ_prun_iterations}
\vspace{-2mm}
\end{figure}

This coding scheme is equivalent to the original scheme, where
$\frac{\lambda_{t-1}}{\lambda_{t}} = \frac{n-1}{n}$ for $1\leq t\leq L$, and 
the codebook $\cC^{(t)}$ consists of $n$-dimensional all-zero vectors except a single nonzero element of value $\frac{1}{\lambda_{t-1}}$. We call our scheme ``successive pruning'' as it can be used to prune NN weights (see Section~\ref{sec:successive}). Algorithm~\ref{algorithm_successive_exp} shows how to implement successive pruning to compress an exponential source sequence, e.g., NN weights, and Figure~\ref{fig:succ_prun_iterations} illustrates how it outputs a sparse vector $\bUh^{(3)}$ by reconstructing $\bU^{(0)}$ iteratively. %We present a simple example of how successive pruning outputs a sparse vector $\bUh^{(3)}$ by reconstructing $\bU^{(0)}$ iteratively in Figure~\ref{fig:succ_prun_iterations}. 
Notice that the encoder needs to send the decoder only an index $i \in \{1, \dots, n\}$ for each iteration. In other words, the encoder does not communicate any continuous variable except the mean of the initial exponential distribution. When there is no index $i$ such that $\bU_i^{(t-1)}\geq \frac{1}{\lambda_{t-1}}$, the encoder re-estimates the empirical mean and sends a refreshed $1/\lambda$ to the decoder. However, this is a rare situation in our experiments ($20$ refreshments in 20M iterations) and hence has a negligible effect on the size of the compressed model. %As can be seen from Figure~\ref{fig:RD_comp}, rate (average number of bits needed to code the indices from first $t$ iterations) and one-sided $\ell_1$ distance between the source sequence and reconstructed sequence are comparable to the theoretical limit in Eq.\ref{eq_rd_exp}.

%The key idea here is that at each iteration $t$, rate (average number of bits needed to code the indices from first $t$ iterations) and one-sided $\ell_1$ distance between the source sequence and reconstructed sequence are comparable to the theoretical limit in Eq.\ref{eq_rd_exp} (see Figure~\ref{fig:RD_comp}).


%In practice, we can make the coding scheme more efficient by estimating $\frac{1}{\lambda_0}$ as the empirical mean. Another practical issue is the possibility that we may encounter a situation where there is no $i \in \{1,\dots,n\}$ such that $\bU^{(t-1)}_i \geq \frac{1}{\lambda_{t-1}}$. In such a case, we recalculate the mean of $\bU^{(t-1)}$ and refresh $\frac{1}{\lambda_{t-1}}$ accordingly. We present our coding scheme in Algorithm~\ref{algorithm_successive_exp} that handles these practical issues as well. Before starting iterative coding, encoder first sends the decoder the empirical mean of the source symbols $\frac{1}{\lambda_{decoder}}$. At each iteration $t$, encoder sends an index $m \in \{1, \dots, n\}$ to the decoder and the decoder is able to reconstruct a sequence given the indices it receives up to $(t-1)$-th iteration. The key point here is that at each iteration $t$, rate (average number of bits needed to code the indices from first $t$ iterations) and one-sided $\ell_1$ distance between the source sequence and reconstructed sequence are comparable to the theoretical limit in Eq.\ref{eq_rd_exp} (see Figure~\ref{fig:RD_comp}).  


%We propose Algorithm~\ref{algorithm_successive_exp} for successively encoding and decoding an $n$-dimensional i.i.d. exponential source $U^{(0)}=(U^{(0)}_1, \dots,U^{(0)}_n )$. 

\subsubsection{Lossless Compression (Entropy Coding)}
\label{entropy_code}
Our coding scheme requires communicating an index $i \in\{1,\dots,n\}$ from the encoder to the decoder for each iteration. %\noa{We do not have to send the message at every iteration, we can store all messages and send them all at the end of final iteration.} 
We need a lossless compression scheme, namely entropy coding, to represent these indices as binary sequences. In information theory, the optimal entropy coding method can be found when the source distribution is known in advance \cite{huffman1952method}. Although there are universal codes that encode any source regardless of the distribution, they are preferable only when the source distribution is unknown since an entropy coding that matches the source distribution is always better than a universal code. Fortunately, our coding scheme for exponential source induces a well-defined distribution that allows us to choose an optimal entropy coding method. Notice that randomly picking an index $i$ from $\{j: \bU^{(t)}_j \geq \frac{1}{\lambda_{t}}\}$ is equivalent to; (1) first randomly permuting $\bU^{(t)}$, and (2) selecting the minimum index $i$ from $\{j: \bU^{(t)}_j \geq \frac{1}{\lambda_{t}}\}$. The second approach induces a geometric  distribution under the i.i.d. assumption on the indices where small indices are always more probable to be selected. For geometric sources, there are two standard entropy coding methods: unary coding and Golomb coding \cite{golomb1966run, gallager1975optimal}. Details about these entropy coding methods are given in Appendix~\ref{entropy_coding_app}. %We evaluate the performance of both methods when they are applied with successive pruning in Figure~\ref{fig:RD_comp}. 
Although both unary coding and Golomb coding show comparable rate distortion trade-off to the rate distortion function in Eq.~\ref{eq_rd_exp}, we use Golomb coding in our experiments. 



%Although both unary coding and Golomb coding show comparable rate distortion trade-off to the rate distortion function in Eq.~\ref{eq_rd_exp}, we use Golomb coding in our experiments since it requires lower rate in low distortion region. 
%\noa{It is bit unclear whether we are in low distortion regime, or high distortion regime.
%If we focus on end-to-end distortion, the distortion is high since we have 90\% pruning.}
%\paragraph{Unary Coding:}
%\paragraph{Golomb Coding:}

\begin{algorithm}[t!]
{\bf Hyperparameters:} scale factor $\alpha$ for empirical mean \\
{\bf Inputs:} exponential sequence $u_1, \dots, u_n$ with $n$ symbols\\
{\bf Output:} reconstructed sequence $u^{recon}_1, \dots, u^{recon}_n$ \\
\vspace{-.2in}
\begin{algorithmic}
\STATE{$(u^{recon}_1, \dots, u^{recon}_n) \gets 0$}
\STATE{$\lambda \gets \mathsf{MeanEst}((u_1,\dots,u_n))$}
\STATE{$\mathsf{Encoder}$ sends $\lambda$ to the $\mathsf{Decoder}$}. 
\FOR{$t=1,\ldots,L$} 
\STATE{\hspace{.15in}\underline{\textbf{Encoder:}}}
\STATE{$m_{inds} \gets$ (indices of the components in $(u_1,\dots,u_n)$ that are larger than $1/\lambda$.)}
\IF{$m_{inds}$ is empty}
\STATE{$\lambda \gets \mathsf{MeanEst}((u_1,\dots,u_n))$}
\STATE{sends $\lambda$ to the $\mathsf{Decoder}$}.
\ENDIF
\STATE $m \gets$ (a random index from $m_{inds}$)
\STATE {sends $m$ to the Decoder.}
\STATE {$u_m = u_m - 1/ \lambda$}
\STATE  {$\lambda\gets \frac{n}{n-1} \cdot\lambda$}\\
\hspace{.15in} \underline{\textbf{Decoder:}}
\STATE {receives $m$ from the Encoder.}
\STATE {$u^{recon}_m = u^{recon}_m + 1/ \lambda$}
\STATE {$\lambda\gets \frac{n}{n-1} \cdot\lambda$}
\ENDFOR \\
\STATE
\STATE $\mathsf{MeanEst}((u_1,\dots,u_n)):$
\STATE \hspace{.15in}{$1/ \lambda \gets$ mean of $(u_1, \dots, u_n)$}
\STATE \hspace{.15in}{$\lambda \gets \alpha \cdot \lambda$}
\STATE \hspace{.15in}{\bf return} $\lambda$  %\noa{is there any reason for an additional indent for return lambda?}
\end{algorithmic}
\caption{Successive Pruning}
\label{algorithm_successive_exp}
\vspace{-1mm}
\end{algorithm}

%   \begin{figure}[h!]
%        \centering %
%        \includegraphics[width=.36\textwidth]{figures/RD-exp_lambda_1.jpg}
%    \caption{Rate-Distortion of Exponential Source. RD:theoretical limit in Eq.~\ref{eq_rd_exp}, Algorithm~\ref{algorithm_successive_exp} with Unary Coding and Algorithm~\ref{algorithm_successive_exp} with Golomb Coding. \berivan{larger legend}}\label{fig:RD_comp}
%    \vspace{-1mm}
%   \end{figure} 

\subsection{Successive Pruning for Model Compression}
\label{comp_NN}
%\noa{The difference between RD and our algorithm is actually not comparable, and even scalar quantization might provide a better RD curve. we may not want to show this figure...}

    
    \begin{figure}[h]
        \centering %
        \subfigure[Sparsity vs Iterations.]{\includegraphics[width=.2383\textwidth]{figures/imagenet_pruning.png}}
        \subfigure[Accuracy vs Iterations. ]{\includegraphics[width=.2383\textwidth]{figures/imagenet_downstream_test_acc.png}}
    \caption{Sparsity and Accuracy of the Reconstructed ResNet-50 on ImageNet. succ. prun.: Successive Pruning.}\label{fig:no_retrain_pruning}
   \end{figure}
   
Finally, we propose successive pruning, a NN compression strategy that combines the iterative coding scheme presented in Algorithm\ref{algorithm_successive_exp} with Golomb coding. Since exponential distribution matches well with the sign-free NN weights, we directly apply Algorithm~\ref{algorithm_successive_exp} to the sign-free weights of a fully-trained NN. We show the accuracy and sparsity of the reconstructed ResNet-50 (on ImageNet) through iterations in Figure~\ref{fig:no_retrain_pruning}. Notice that the sparsity in the reconstructed weights is $100\%$ at the first iteration, and it decreases as the decoder receives new indices from the encoder (as in Figure~\ref{fig:succ_prun_iterations}). As the iterations proceed, we are able to recover the accuracy of the original model (see Figure~\ref{fig:no_retrain_pruning}(b)).% after some iterations.
   % \vspace*{-.2cm}

   

   
  % \noa{Figure 6 is bit confusing, how about having a feedback that shows ``iteratively applying successive pruning and retraining'', then apply entropy coding, etc.}

 Retraining the pruned model to tune the non-pruned weights is a widely accepted procedure, and it usually boasts the accuracy in higher compression ratios. We adopt this approach by running successive pruning in two phases, as shown in Figure~\ref{fig:pruning_diagram}. In phase-$1$, we apply successive pruning to the non-pruned weights $w$ until we reach a desired sparsity $s$ (sparsity is always non-increasing, see Figure~\ref{fig:no_retrain_pruning}(a)). Once we get the sparsity $s$, we stop the successive pruning algorithm and construct a pruning mask $\mathcal{M}_p \in\{0,1\}^n$ based on the nonzero elements' locations in the reconstructed weight $\hat{w}$, i.e., if $\hat{w}_i > 0$, then $\mathcal{M}_{p,i}=1$. We use $\mathcal{M}_p$ to prune the original weights $w$, i.e., $w_{\text{pruned}}=\mathcal{M}_p \odot w$.
 %\st{We tune the nonzero weights of $w_{\text{pruned}}$ by training it for a few epochs. We call the retrained $w_{\text{pruned}}$ as $w_{\text{retrained}}$. }\noa{retrained weight with initial weight $w_{retrained}$, and fix zeros (pruned weights) while training} \berivan{I couldn't understand what you mean here} \noa{I think the definition of $w_{retrained}$ is bit unclear.}
 %\wip{How about :
 %From weights $w_{pruned}$, we retrain the nonzero parameters for few epochs,
 %and call the the retrained weights by $w_{retrained}$.}
 From the weights $w_{\text{pruned}}$, we retrain the nonzero ones for a few epochs and call the retrained weights by $w_{\text{retrained}}$.
 After resetting the reconstructed weights $\hat{w} =0$,  we start phase-$2$. During phase-$2$, we apply successive pruning to $w_{\text{retrained}}$ which has sparsity $s$. At the end of phase-$2$, we have a reconstructed weight $\hat{w}$ whose sparsity is lower bounded by $s$. In short, phase-$1$ outputs a pruning mask that is used to prune the model whereas phase-$2$ is devoted to finding the binary representation of the pruned and retrained model. With this $2$-phase approach, successive pruning consistently outperforms existing pruning strategies in terms of accuracy-sparsity trade-off (output of retraining in Figure~\ref{fig:pruning_diagram}), and we achieve a comparable (mostly better) compression rates (output of phase-$2$ in Figure~\ref{fig:pruning_diagram}). Since we apply the successive pruning algorithm to a retrained pruned model in phase-$2$, we need an exponential distribution over weights of this model as well. We verify that exponential distribution is still a good fit for retrained model's nonzero and sign-free weights through density plots in Appendix~\ref{succ_pruning_app}. %Notice that we need an exponential distribution over the sign-free weights of the retrained sparse model since we apply successive pruning algorithm to it in phase-$2$. We show that the sign-free NN weights after pruning and retraining still follow an exponential distribution  
 
 %we are comparable to (mostly better than) existing strategies \cite{deep_compression, molchanov2017variational, snip, tartaglione2018learning, woodfisher, hydra} in terms of accuracy-sparsity, and we outperform them in the binary representation length. 

     \begin{figure}[h!]
        \centering %
        \includegraphics[width=.47\textwidth]{figures/succ_refin_pruning.png}
    \caption{End-to-End NN Compression with Successive Pruning.}\label{fig:pruning_diagram}
   \end{figure}
   
   %\vspace*{-.2cm}
   
 %\noa{How about having subsection (or another section) for comparison / discussions?}

 Successive pruning differs from the existing pruning and encoding methods in the way how the pruned model is encoded. \cite{deep_compression} propose iterative magnitude pruning with retraining to find the pruning mask $\mathcal{M}_p$ (phase-$1$ and retraining). After the pruned model $w_{\text{pruned}}=\mathcal{M}_p \odot w$ is constructed, they represent this model as a list of tuples $(i,w_i)$, where $i$ and $w_i$ are the location and value of a nonzero weight. They use compressed sparse row (CSR) or compressed sparse column (CSC) formats to efficiently code the relative indices $i-j$, where $j$ is the index of the previous nonzero weight. They put a limit for the maximum allowable relative index to keep the bit representation shorter. If there are no nonzero weights in the range, the encoder puts a filler zero. Since each weight $w_i$ is a $32$-bit floating-point, they quantize $w_i$'s to represent weights more efficiently. Lastly, they apply Huffman coding for both relative indices $i-j$ and weights $w_i$ \cite{huffman}. There are three main problems with this approach: (1) the trick with filler zeros to limit the number of bits per relative index is inefficient for high sparsity ratios, (2) quantization of the weights brings additional accuracy loss and requires extra tuning steps, and (3) the distribution used for Huffman coding needs to be encoded as well. \cite{DeepCABAC} do not propose a new pruning framework but show promising results with context-aware binary arithmetic coding (CABAC) in encoding a pruned model \cite{CABAC}. That is, they take a retrained pruned model and encode it via CABAC (phase-$2$). While both \cite{deep_compression} and \cite{DeepCABAC} encode a pruned model in a lossy way, our method directly applies Golomb coding to the output of successive pruning algorithm (geometrically distributed indices). In other words, our end-to-end compression method has three advantages over the existing approaches: (a) it does not require an additional lossy and costly step such as quantization before encoding, (b) it only encodes discrete-valued indices instead of floating points (e.g., weight values), and (c) the entropy coding method perfectly matches the predefined distribution of the indices, i.e., it is optimal.
% \noa{It seems this paragraph focuses on compression after the pruning (instead of pruning method itself).}
 
 We underline that successive pruning can be combined with other pruning or encoding strategies. As shown in Figure~\ref{fig:pruning_diagram}, we can use any pruning strategy in phase-$1$ and encode the pruned model with successive pruning in phase-$2$, or we can use successive pruning in phase-$1$ as a pruning framework and encode the pruned model with other methods such as CSR+quantization+Huffman and CABAC.  
 %\noa{Successive pruning in phase-2 is confusing. How about using the term ``successive refinement'' if we are using the same technique in phase-2?}
 
% What makes successive pruning fundamentally different from the prior work is the way we code the pruned model. As previously mentioned, conventional pruning techniques search for weights to be pruned, i.e. they learn a pruning mask, although they differ in the criterion to determine whether a weight should be pruned or not %\cite{han2015learning,deep_compression,hydra, woodfisher}
% . After finding a pruning mask $\mathcal{M}_p \in \{0,1\}^n$, they use it to prune the model as $\hat{w} = \mathcal{M}_p \odot w$. In order to find a binary representation of the pruned model, i.e. encode $\hat{w}$, \cite{deep_compression} propose first representing the location of nonzero elements of $\hat{w}$ in CSR or CSC formats, and then encode these representations and weight values using Huffman coding \cite{huffman}. Encoding the sparse locations of non-pruned weights is costly as CSR and CSC formats do not capture the statistics of NN weights. Likewise, encoding the weight values without aggressive quantization and tuning is costly as weights are in $32$-bit floating point format. In successive pruning, we do not need to encode the sparse locations or the values of the non-pruned weights to represent $\hat{w}$. All we need to encode is the mean of the weight magnitudes (one $32$-bit floating point) and a list of indices (one index per iteration) which has a geometric distribution (see Section~\ref{entropy_code}). As explained in Section~\ref{entropy_code}, these geometrically distributed indices can be encoded via Golomb coding optimally. We achieve to represent the same pruned model with $10$ times less number of bits than the prior work thanks to our joint pruning-encoding scheme. \\    


 
%\begin{algorithm}
%{\bf Hyperparameters:} scale factor for empirical mean $\alpha$ \\
%{\bf Inputs:} weights of a fully trained neural network $w_{in}$\\
%{\bf Output:} reconstructed weights $w_{recon}$ \\
%\vspace{-.2in}
%\begin{algorithmic}
%\State{$w_{res} \gets w_{in}$}
%\State{$w_{recon} \gets 0$}
%\State{$\lambda \gets$ mean of $w_{res}$}
%\State{$\lambda_{scaled} \gets \alpha \cdot \lambda$} \\
%\For{$t=0,\ldots,T-1$}
%\State{$m \gets  \mathsf{Encoder}(w_{res}, \ \lambda_{scaled})$}
%\While{$m$ is None}
%\State{$\lambda \gets$ mean of $w_{res}$}
%\State{$\lambda_{scaled} \gets \alpha \cdot \lambda$}
%\State{$m \gets  \mathsf{Encoder}(w_{res}, \ \lambda_{scaled})$}
%\EndWhile
%\State{$w_{res}[m] = w_{res}[m] - \lambda_{scaled}$}
%\State{$w_{recon}[m] = w_{recon}[m] + \lambda_{scaled}$}
%\State{$\lambda_{scaled}\gets \frac{n-1}{n} \cdot\lambda_{scaled}$}
%\EndFor \\
%\State $\mathsf{Encoder}(w_{res},  \ \lambda_{scaled}):$
%\State \hspace{.15in} $m_{inds} \gets$ (indices of the components in %$w_{res}$ that are larger than $\lambda_{scaled}$.)
%\State \hspace{.15in} {\bf if}{ length of $m$ is $0$}{ \bf then:}
%\State \hspace{.45in} {\bf return} None
%\State \hspace{.15in} {\bf end if}
%\State \hspace{.15in} $m \gets$ (a random index from $m_{inds}$)
%\State \hspace{.15in} {\bf return} m
%\end{algorithmic}

%\caption{Successive Pruning }
%\label{algorithm_successive_pruning}
%\end{algorithm}

%\noa{agreed}
%\berivan{be explicit about the following: successive pruning is an end-to-end compression method. but it can be combined with other strategies as well:
%\begin{itemize}
%    \item first phase outputs a pruning mask. we can use it as a pruning framework and apply quantization+huffmancoding(\cite{deep_compression} with CSR format, or we can apply DeepCABAC\cite{DeepCABAC} to find the binary respresentation)
%    \item second phase takes a pruned network and finds its binary respresentation. Any pruned network (\cite{deep_compression} etc) can be an input to the second phase.
%\end{itemize}}


\subsection{Compression for Federated Learning}
\label{fl}
In this section, we point another compression problem that can benefit from successive pruning strategy. In federated learning, a NN model is trained across multiple edge devices, each having local training data \cite{federated1}. %The idea is to keep local data at the edge to preserve the user privacy. 
Each device is responsible for doing some local training over the local data and sending the local gradients %(which are assumed to leak no information about the local data) 
to a centralized processor. The communication of gradients at each round is costly as the gradients are in model size. Given the resource limitations of edge devices, gradient communication is a significant bottleneck in federated learning, and gradient compression is crucial \cite{federated2}. 

We present density plots of gradients in Appendix~\ref{fl_app}, supporting that Laplacian distribution is a good fit for NN gradients during different stages of the training, and exponential distribution almost perfectly matches the distribution of sign-free gradients. %This suggests that reconstructed gradients are sparse in the rate distortion theoretic optimal gradient compression scheme. 
%rate distortion theoretic optimal gradient compression scheme gives a sparse reconstruction.
Following the same reasoning in model compression, %rate distortion theoretic optimal gradient compression scheme gives a sparse reconstruction and 
we propose the successive pruning strategy for compressing the sign-free gradients in federated learning. %Similar to NN compression problem, reconstructed gradients in the centralized processor are sparse by rate distortion theory.
Similar to the case in pruning, existing sparsification methods for local gradients do not propose an efficient encoding scheme for sparsified gradients \cite{lin2017deep, federated0,Aji,Wang, Wangni, barnes2020rtop}. %rather than a naive encoding of the nonzero gradients' locations which requires $k \log n$ bits where $k$ is the number of nonzero gradients and $n$ is the number of all gradients
%Our strategy is most similar to \cite{barnes2020rtop} in that they also do a random selection among the largest gradients. 
%although they study the communication-efficient federated learning problem from a statistical mean estimation approach as opposed to our rate distortion theoretic approach.
%in that they also randomly select gradients among the largest ones. 
%However, their random selection is uniform whereas our strategy attains higher probability for larger gradients to be selected due to iteratively decreasing threshold ($\frac{1}{\lambda}$). %It is still worth noting that these two strategies are similar although  rTop-$k$ approaches the problem from a statistical mean estimation approach in contrast to our information-theoretic approach. 
 With successive pruning, we provide a novel gradient  sparsification strategy followed by Golomb coding that requires an order of magnitude less communication budget to send the compressed gradients compared to prior work.  



%As can be seen from Figure~\ref{fig:density_grad}, Laplacian distribution is a good fit for NN gradients and, as expected, exponential distribution almost perfectly matches the sign-free gradients. Following the same reasoning that we use for NN compression, we propose successive pruning strategy for compressing the sign-free gradients in federated learning.

%The sparsification of gradients for federated learning is first proposed by \cite{lin2017deep}. Among several sparsification strategies \cite{ federated0,Aji,Wang, Wangni}, rTop-$k$ \cite{barnes2020rtop} is the most similar one to successive pruning, in that they also perform a random selection over the gradients larger than a threshold. %They model the gradients as a sparse bernoulli random vector and prove the optimality of their strategy by formulating the problem as a statistical mean estimation problem. On the other hand, we make a more realistic assumption over the gradient distribution and interestingly reach the same conclusion: random selection over the large gradients. 
%However, similar to the case in pruning, none of the existing sparsification strategies, including rTop-$k$, perform an efficient encoding of the sparsified gradients. Our initial experiments suggests that successive pruning provides an order of magnitude more efficient encoding of the sparsified gradient vector compared to \cite{lin2017deep, barnes2020rtop}. 

 %\berivan{clean federated learning section up.}


   

   


==> sections/04-experiments.tex <==
\section{Experiments}
\label{experiments}

\begin{figure*}[t!]
        \centering %
        \subfigure[ResNet-50 on ImageNet.]{\includegraphics[width=.40\textwidth]{figures/comparison_resnet50.png}}
        \subfigure[ResNet-18 on CIFAR-10. ]{\includegraphics[width=.40\textwidth]{figures/comparison_resnet18.png}}
        \subfigure[Small VGG-16 on CIFAR-10 (10-94 $\%$ Accuracy). ]{\includegraphics[width=.40\textwidth]{figures/comparison_vgg16_retraining_full.png}}
        \subfigure[Small VGG-16 on CIFAR-10 (92-94 $\%$ Accuracy). ]{\includegraphics[width=.40\textwidth]{figures/comparison_vgg16.png}}
    \caption{Comparison of Mag. Prun.: magnitude pruning \cite{deep_compression}; Succ. Prun. (phase 1): successive pruning in phase-$1$+retraining; Succ. Prun. (phase 1$\&2$): successive pruning in phase-$1$+retraining+successive pruning in phase-$2$. Successive pruning experiments are conducted $3$ times.}\label{fig:comp_weight}
   \end{figure*}
We present successive pruning results in Section~\ref{exp_succ_pruning}, and some preliminary results on compression for federated learning in Section~\ref{exp_fl}. We ran the experiments $3$ times as our method involves random permutation and selection. %For conciseness, we give the average numbers in the main body of the paper and refer the reader to Appendix~\ref{exp_app} for more detailed results with confidence intervals.

%\paragraph{Datasets and Models:} 
We consider three image datasets: MNIST \cite{lecun2010mnist}, CIFAR-10 \cite{krizhevsky2009learning} and ImageNet \cite{imagenet_cvpr09}. %We use the standard train/val/test splits for both, and for CIFAR-10 we apply random horizontal flips as data augmentation during training.
For the MNIST experiments, we use two architectures: LeNet-5-Caffe, and LeNet-300-100 \cite{lecun1998gradient}. For CIFAR-10, we use two architectures: ResNet-18 \cite{he2016deep} and small VGG-16 \cite{vgg}. For ImageNet, we use pretrained ResNet-50 from PyTorch \cite{he2016deep, NEURIPS2019_9015}. We give additional details on model architectures and hyperparameters in Appendix~\ref{hyperparams}. %\noa{How about using ``\mbox{\textbackslash appendix}'' to use Section alphabet instead of Section number for Appendix.}

%For the MNIST experiments, we use two architectures: LeNet-5-Caffe (431K params), and LeNet-300-100 (267K params) \cite{lecun1998gradient}. For CIFAR-10, we use two architectures: ResNet-18 (11.2M params) \cite{he2016deep} and small VGG-16 (14.7M params) \cite{vgg}. For ImageNet, we use pretrained ResNet-50 (25.6M params) from PyTorch \cite{he2016deep, NEURIPS2019_9015}. We give additional details on model architectures and hyperparameters in Appendix~\ref{hyperparams}.

\subsection{Model Compression}
\label{exp_succ_pruning}

   
For the accuracy-sparsity trade-off, we compare our scheme with magnitude pruning \cite{deep_compression} since \cite{frankle2020pruning} show that magnitude pruning performs better than many alternative pruning frameworks \cite{snip, frankle2018lottery,wang2020picking, tanaka2020pruning}. For both successive pruning and magnitude pruning, we retrained the pruned model for $20$ epochs. Although we applied one-shot pruning, i.e., prune once and retrain once, for both methods, it is straightforward to extend successive pruning with several phase-$1$'s followed by one phase-$2$ to perform iterative pruning with increasing sparsity ratios. We show in Figure~\ref{fig:comp_weight} that successive pruning consistently achieves better test accuracy than magnitude pruning under the same sparsity constraint on ImageNet and CIFAR-10 datasets with ResNet-50, ResNet-18, and small VGG-16. We present additional results on MNIST with LeNet-5-Caffe and LeNet-300-100 in Appendix~\ref{exp_app}. The improvement of successive pruning is more evident in higher sparsity ratios. For instance, magnitude pruning with $95\%$ sparsity results in $10\%$ test accuracy (random prediction) for VGG-16 on CIFAR-10, whereas successive pruning achieves $90\%$ accuracy with the same sparsity (see Figure~\ref{fig:comp_weight}(c)). 

\setlength{\tabcolsep}{3pt}
\begin{table}[h!]
%\vspace{-1mm}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{cccccc}
\toprule
Model              & Original         & Method        & Sparsity                      & Comp.       &Comp.\\ 
(Original size)    & Acc. ($\%$)     &               &  $\frac{|w =0|}{|w|} (\%)$       & Size           & Acc. ($\%$)\\ \midrule
 \centered{
    LeNet-5-Caffe  \\
    MNIST\\
    (1.72 MB)}     &\centered{99.1} &\centered{Deep Comp.\\
                                        DNS \\
                                        SWS \\
                                        DeepCABAC \\
                                        Succ. Prun.(1\&2) \\
                                        Succ. Prun.(1\&2)}    & \centered{92.0 \\
                                                                    99.1 \\ 
                                                                    99.5 \\ 
                                                                    98.1 \\ 
                                                                    99.2 \\
                                                                    99.3}           & \centered{44 KB ($\times 39$)\\
                                                                                                16 KB ($\times 107$) \\
                                                                                                11 KB ($\times 156$) \\
                                                                                                12 KB ($\times 143$) \\
                                                                                                \textbf{7 KB ($\times 246$)}\\
                                                                                                \textbf{5 KB ($\times 344$)}}     & \centered{99.3\\
                                                                                                                                                99.1 \\
                                                                                                                                                99.0 \\
                                                                                                                                                99.1 \\
                                                                                                                                                99.0 \\
                                                                                                                                                98.0}  \\ \midrule
\centered{LeNet-300-100 \\
MNIST \\
(1.06 MB)}        & \centered{98.6}      &\centered{Deep Comp. \\
                                                    SWS\\
                                                    DeepCABAC \\
                                                    Succ. Prun.(1\&2) \\
                                                    Succ. Prun.(1\&2)}    &\centered{92.0 \\
                                                                                95.7\\
                                                                                91.0    \\
                                                                                96.5 \\
                                                                                 98.0    }               & \centered{27 KB ($\times 40$) \\
                                                                                                                16.7 KB ($\times 64$)  \\
                                                                                                                19.4 KB ($\times 54$) \\
                                                             \textbf{14.8 KB ($\times 72$)}  \\                   \textbf{6.9 KB ($\times 155$)}}              & \centered{98.4 \\
                                                                                                                                                                    98.1  \\
                                                                                                                                                                    98.0 \\
                                                                                                                98.1 \\                                             97.1  }\\  \midrule
%\centered{ResNet-18 \\
%CIFAR-10  \\
%(44.70 MB) }        &\centered{95.60 }       &\centered{Succ. Prun. \\
%                                                        Succ. Prun. \\
%                                                        Succ. Prun.}    &\centered{90.0 \\
%                                                                                    95.0 \\
%                                                                                    97.0}        &\centered{3.1 MB ($\times 15$) \\
%                                                                                                            1.1 MB ($\times 42$) \\
%                                                                                                            \textbf{875 KB ($\times 53$)}}              &\centered{ 95.1\\
%                                                                                         92.2 \\
%                                                                                        90.0 }\\ \midrule
%\centered{Small VGG-16 \\
%CIFAR-10 \\
%(58.91 MB)}                &\centered{93.60}        &\centered{DeepCABAC \\
%                                                             Succ. Prun.\\
%                                                             Succ. Prun.}     &\centered{92.4 \\
%                                                                                          95.0 \\
%                                                                                          90.0 }   &\centered{956 KB ($\times 61$) \\
%                                                                                                        \textbf{1.1 MB ($\times 54$)}\\
%                                                                                                        3.0 MB  ($\times 20$)}                      &\centered{91.0 \\
%                                                                                                                                                            91.1 \\
%                                                                                                                                                            93.0 } \\ \midrule
\centered{ResNet-50 \\
        ImageNet \\
        (102.23 MB)  }         & \centered{76.6}     & \centered{Deep Comp. \\
                                                            DeepCABAC \\
                                                            Succ. Prun.(1\&2) \\
                                                            Succ. Prun.(1\&2) \\
                                                            Succ. Prun.(1)}         & \centered{71.0 \\
                                                                                          74.6 \\
                                                                                          90.0  \\ 
                                                                                          70.0 \\
                                                                                          71.0 }                   & \centered{6.1 MB ($\times 16$) \\
                                                                                                                                6.1 MB ($\times 16$) \\
                                                                                                                                 7.5 MB ($\times 13$) \\
                                                                                                                                 17.3 MB ($\times 6$) \\
                                                                                                                                 \textbf{6.1 MB ($\times 16$)}}           & \centered{76.1 \\
                                                                                                                                                                                74.1 \\
                                                                                                                                                                                70.2 \\
                                                                                                                                                                                74.6\\
                                                                                                                                                                                74.6} \\
\bottomrule
\\
\end{tabular}
}
\caption{Comparison of Successive Pruning with Other Pruning Strategies in terms of Accuracy, Sparsity and Size. Succ. Prun.(1\&2): Successive Pruning in both phases; Succ. Prun.(1): Successive Pruning in phase-$1$ + CSR and Huffman in phase-$2$; Deep Comp.: \cite{deep_compression}; DNS: \cite{guo2016dynamic}; SWS: \cite{ullrich2017soft}; DeepCABAC: \cite{DeepCABAC}.
}
\label{tab:comparison}
\end{table}
%\vspace{-5mm}


We also compare successive pruning with Deep Compression \cite{deep_compression}, Dynamic Network Surgery \cite{guo2016dynamic}, Soft Weight Sharing \cite{ullrich2017soft}, and DeepCABAC \cite{DeepCABAC} in terms of pruned model's size %\noa{memory size sounds like memory usage(RAM) while running compression algorithm. I prefer the size of compressed file (or similar), but if ``memory size'' is a common term in this field, you can keep it. } 
in Table~\ref{tab:comparison}. For conciseness, we give the average numbers over $3$ runs and refer the reader to Appendix~\ref{exp_app} for more detailed results ($5$ architectures, $3$ datasets) with confidence intervals. %Notice that successive pruning can preserve the original accuracy on MNIST even with high sparsity ratios ($99.2\%$ for both LeNet-5-Caffe, $98\%$ for LeNet-300-100. Furthermore the size of the model is reduced by $344$ and $155$ times for LeNet-5-Caffe and LeNet-300-100, respectively, which is $2.5$ times more memory-efficient than the previous work.
Notice that successive pruning reduces the model size by $344$ and $155$ times for LeNet-5-Caffe and LeNet-300-100 while still preserving the original accuracy on MNIST. This is an improvement by $2.5$ times in the compression rate compared to the previous work.
However, for ResNet-50, the memory efficiency that successive pruning provides is not higher than the previous work. We believe that this is due to the different sparsity levels between MNIST and ImageNet tasks.
For the moderate sparsity levels, e.g.,~$71\%$ in ResNet-50, CSR representation in \cite{deep_compression} is efficient with three tricks: (1) the encoder encodes the relative index between nonzero weights instead of actual indices, (2) there exists a maximum span of relative indices, and (3) the encoder inserts a filler zero when there is no nonzero weight to be encoded in the allowed span.
%However, to keep the bit representation shorter, there exists a maximum allowable relative index.
%If there are no nonzero weights in the range, the encoder puts a filler zero.
These tricks lead to inefficient encoding when the sparsity ratio is high, e.g.,~LeNet-5-Caffe with $99\%$ sparsity,
because it requires either (i) a larger span of the relative indices with more bits per index, or (ii) additional redundant filler zeros.
%it requires the broader  with more bits per index, or additional redundant filler zeros.
Thus, after applying successive pruning in phase-$1$; our procedure for phase-$2$ is to (a) apply successive pruning when the model sparsity is high, and (b) apply CSR representation with Huffman coding \cite{deep_compression} or DeepCABAC \cite{DeepCABAC} when the model sparsity is low.
The last row of Table~\ref{tab:comparison} shows that successive pruning in phase-$1$
followed by CSR representation and Huffman coding in phase-$2$ outperforms previous work in accuracy-size trade-off.

%\noa{Instead the following green texts how about the following blue texts? \\ Our explanation for this is different sparsity levels used in MNIST and ImageNet tasks.
%When the sparsity is not too high, e.g. $71\%$ in ResNet-50, CSR representation in \cite{deep_compression} is efficient because they only code the relative index between nonzero weights by putting a limit on the maximum relative index to keep the bit representation shorter.
%When there is no nonzero weight in their limited span, they put a filler zero.
%Notice that this representation is not efficient with high sparsity ratios, e.g. $99\%$ sparsity in LeNet-5-Caffe, because we need to either (i) increase the limit of the relative indices which requires greater number of bits per index, or (ii) put many filler zeros.
%Motivated by this observation, for the phase-$1$ we propose successive pruning since it is better than previous work in accuracy-sparsity trade-off,
%and for the phase-$2$, successive pruning in high sparsity regime and CSR representation with Huffman coding \cite{deep_compression} or DeepCABAC \cite{DeepCABAC} in low sparsity regime might be a good option.

%As can be seen from the last row of Table~\ref{tab:comparison}, successive pruning in phase-$1$ followed by CSR representation and Huffman coding in phase-$2$ outperforms previous work in accuracy-memory size trade-off.}

%When the sparsity is high, e.g. $99 \%$ for LeNet-5-Caffe, Deep Compression (CSR representation combined with quantization and Huffman coding) is costly \cite{deep_compression}. The reason is,  
We consider the approaches of \cite{oktay2019scalable, havasi2018minimal} %to find the minimum representation of a model 
orthogonal to our work %and do not compare our results with them 
for two reasons: (1) they modify the training process, which is different from our problem of compressing any given trained model,
%\st{and (2) their reconstructed model is not sparse and hence does not enjoy faster computation.}
and (2) their reconstruction is not sparse while our primary focus is a sparse representation that provides faster computation.
%\noa{CAN WE MOVE THIS TO INTRODUCTION? that we are not considering nonsparse compression schemes.}

%\berivan{we do not compare our results with \cite{oktay2019scalable, havasi2018minimal} that can achieve higher memory-efficiency since they do not reconstruct a sparse model and modify the training process which brings a huge complexity. thus lack the benefits of pruning.
%}
%\berivan{\cite{frankle2020pruning} show that magnitude pruning after training outperforms pruning at initialization methods \cite{snip, wang2020picking, tanaka2020pruning}.}






%\paragraph{MNIST:}
%\paragraph{CIFAR-10:}
%\paragraph{ImageNet:} 

\subsection{Compression for Federated Learning}
\label{exp_fl}
In our preliminary experiments on federated learning of LeNet-5-Caffe on MNIST with $10$ devices, we compare successive pruning with Deep Gradient Compression (DGC) \cite{lin2017deep} which communicates the top-$k$ largest gradients and rTop-$k$ \cite{barnes2020rtop} which communicates randomly selected $k$ gradients among the largest $r$ gradients.
%\st{We compute the size of the sparse gradients for prior work by assuming a naive encoding with $k \log n$ bits where $n$ is the number of parameters in the model as there is no other encoding method proposed for sparse gradients.}
We compute the communication budget for prior work by assuming a naive encoding with $k(\log n+32)$ bits ($n$ is the number of model parameters)
since no efficient encoding method is provided.
With the same sparsity ratio $99.9 \%$, DGC achieves $98.5\%$ accuracy with $2.05$KB of budget, rTop-$k$ achieves $99.1 \%$ accuracy with $2.05$KB of budget, and successive pruning achieves $99.1\%$ accuracy with $218$B  of budget. Thus, successive pruning provides an order of magnitude improvement in the gradients' compression rate while achieving the same accuracy as rTop-$k$. 

==> sections/05-related.tex <==
\section{Related Work}
\label{related}
\berivan{If we have space:
\begin{itemize}
    \item representing NNs in minimum number of bits. Previous work does this but their reconstructed model is not sparse. thus lack the benefits of pruning.
\end{itemize}
If we don't have space, mention related work in the main body as much as possible
}

==> sections/06-discussion.tex <==
\section{Discussion}
\label{discussion}


